MegaScale-Omni: A Hyper-Scale, Workload-Resilient System for MultiModal LLM Training in Production

As the foundational component of versatile AI applications, training an multimodal large language model (MLLM) relies on multimodal datasets with dynamic modality mixture proportions and sample length distributions. However, existing MLLM systems remain inefficient under dynamic workloads, due to statically coupled decisions of resource allocation and model parallelization between encoders and the LLM backbone. This paper presents MegaScale-Omni, an industrial-grade MLLM training system tailored for dynamic workload adaption and hyper-scale deployment. MegaScale-Omni is built upon the training scheme of encoder-LLM multiplexing with three key innovations: (1) Decoupled parallelism strategies with long-short sequence parallelism for encoders to process variable-length samples, and full-fledged 5D parallelism for the LLM backbone, both organized under a communication-efficient parallelization layout. (2) Unified encoder-LLM representations for flexible, extensible colocation, and a new paradigm of encoder-LLM joint pipeline with workload resilience. (3) Workload balancing techniques via decentralized grouped reordering in data loaders and adaptive resharding from encoder to LLM ranks. MegaScale-Omni is deployed as the foundation of our in-house large-scale MLLM training tasks with thousands of GPUs. Our experimental results demonstrate $1.27\times$-$7.57\times$ throughput improvement under production-grade dynamic workloads, as compared to four state-of-the-art systems.

==> contents/discussion.tex <==
\section{Discussion}\label{sec:discussion}


==> sections/approach.tex <==
\section{Approach}

%\subsection{Hello World}

==> sections/experiments.tex <==
\section{Experiments}

%\subsection{Hello World}


\section{Conclusion}

==> sections/introduction.tex <==
\section{Introduction}\label{sec:intro}

Multimodal large language models (MLLMs) have become a foundational component for general-purpose artificial intelligence. 
By encoding heterogeneous modality data as the input to a large language model (LLM), MLLMs extend the capabilities of text-based models to additional modalities such as image~\cite{vit}, audio~\cite{usm}, and video~\cite{video_swin}. 
These models have achieved notable progress across a range of applications~\cite{seed1.5-vl,qwen2-vl,step_audio,gpt4o,gemini1.5}, including content generation, embodied intelligence, and visual understanding. 
Architecturally, an MLLM consists of an LLM backbone together with a set of modality-specific encoders, decoders, and adapters, as depicted in Figure~\ref{fig:mm_arch}(a).
The training data of each modality is first processed by its corresponding encoder to generate unified embeddings, then concatenated as the input to the LLM backbone, as shown in Figure~\ref{fig:mm_arch}(b).
% As illustrated in the ~\autoref{fig:mm_arch}, input data from each modality is first processed by its corresponding encoder, and the resulting embeddings are concatenated to form the input to the LLM backbone.




%Multimodal large language models (MLLMs) have recently emerged as a foundational class of architectures for general-purpose AI applications, enabling capabilities such as real-world perception, reasoning, and content generation\cite{seed1.5-vl,qwen2-vl,step_audio,gpt4o,gemini1.5}. Unlike text-only LLMs, MLLMs integrate multiple modalities—such as images~\cite{vit}, audio~\cite{usm}, and video~\cite{video_swin}—through modality-specific encoders connected to a shared LLM backbone, thereby extending large-scale language modeling to multimodal domains.

\begin{comment}
Multimodal large language models (MLLMs) have emerged as a transformative foundation for general-purpose AI applications, featuring real-world understanding, reasoning, and generation~\cite{seed1.5-vl,qwen2-vl,step_audio,gpt4o,gemini1.5}.
They break the limitations of text-only LLMs by integrating diverse modalities, including image~\cite{vit}, audio~\cite{usm}, and video~\cite{video_swin}, into a unified architecture with modality-specific encoders, an LLM backbone, and decoders (listed in processing order).
To leverage these powerful models, Model as a Service (MaaS) providers train and deploy in-house MLLMs as backends for versatile scenarios, such as vision understanding~\cite{vlm_survey} and generation~\cite{mogao}.
% vision-language~\cite{vlm_survey} and visual understanding and generation~\cite{mogao}.
% such as multimodal dialogue~\cite{chatgpt} and video generation~\cite{veo3}.

% \chunyu{Try add a figure, emphasise industrial elements, refer to PipeWeaver.}
\end{comment}



% From our experience, industrial MLLM training demonstrates \textit{dynamic workloads} on encoders and the LLM backbone, stemming from two major causes.

Unfortunately, the training efficiency of existing MLLM systems remains limited in production environments.
From our experience with large-scale, real-world MLLM training, we identify that the main obstacle lies in \textbf{the dynamic variation of relative workloads between encoders and the LLM backbone throughout training.}
% the main obstacle is that \textbf{the relative workloads of encoders and the LLM backbone vary dynamically over the training process}.
% The sources of this dynamism primarily lie in two factors: the {\it dynamic proportion of modality data} and the {\it variability in multimodal input sample lengths}. 
This dynamism stems primarily from two factors: the {\it dynamic modality data ratios} and the {\it variability in multimodal input sample lengths}. 


Specifically, to attain balanced model capability across modalities, MLLM training is typically divided into multiple phases, each with distinct ratios of modality-specific data~\cite{seed1.5-vl,internlm,qwen2.5-vl}.
Figure~\ref{fig:intro}(a) presents a multi-phase training recipe for a Vision-Language Model (VLM).
The process begins with a pretraining phase, where the LLM and Vision Transformer (ViT)~\cite{vit} are separately trained on text and image data, respectively. 
Then, in phase P0, adapters are trained on image and video data while the LLM and ViT remain frozen.
In subsequent phases, researchers carefully adjust the ratios of both modalities and task domains to balance the model capability when training the entire MLLM.
% model capability when training the entire MLLM.
Some approaches further adapt modality data ratios smoothly throughout these phases, such as every one or a few steps, while the research community continues to explore more dynamic multimodal data mixing strategies.
% continuously and smoothly adapt the modality data proportion throughout these phases, such as every one or a few training steps, while researchers keep seeking more dynamic multimodal data mixtures.
% Accordingly, the workloads of encoders and the LLM backbone evolve as training progresses.
Accordingly, the relative workloads of encoders and the LLM backbone shift continuously as training proceeds.
% For example, in phase P2 with $54\%$ images, the image encoder requires additional compute resources \textcolor{blue}{to maintain consistent encoding latency}.


\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/intro/mm_arch.pdf}
\vspace{-6mm}
\caption{Multimodal LLM architecture and data processing.}
\label{fig:mm_arch}
\vspace{-1mm}
\end{figure}


\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/intro/intro.pdf}
\vspace{-6mm}
\caption{Dynamic workloads in hyper-scale MLLM training and resulting throughput degradation in existing systems.}
\label{fig:intro}
\vspace{-2mm}
\end{figure}


% For example, in Stage P2, where the fraction of image data is higher, the image encoder typically demands additional computational resources. %Figure~\ref{fig:intro}(c) reports the throughput of a 128-GPU Megatron training workload under varying modality ratios. The results show that throughput can differ by up to 2.84× across different dataset compositions. 


In addition, mixing datasets across modalities and task domains exacerbates the skewness of sample length distribution in training batches.
Figure~\ref{fig:intro}(b) reports statistics for two datasets with image-text pairs.
As observed, significant disparities exist not only across modalities (e.g., 1K/3.8K for average text/image lengths) but also across datasets of the same modality (e.g., $2.71\times$ for image length). 
When mixing audio and text datasets, the average difference reaches up to $17.6\times$ (Figure~\ref{fig:intra_modality}). 
Such disparities lead to workload imbalance for encoders either across modalities or within the same modality, ultimately degrading the training efficiency.


% In addition, multimodal inputs exacerbate the skew in sequence length distributions, also leading to variability in the computational loads of both the encoders and the LLM backbone. 
% Figure~\ref{fig:intro}(b)  presents the sequence length distributions of different multimodal datasets. 
% As shown, substantial shifts exist not only across modalities but also among datasets within the same modality, with maximum input lengths differing by up to xx. 
% Such disparities in sequence length can create imbalances in the workload of encoders—either across modalities or among replicas of the same encoder—ultimately degrading overall training performance. 

%Unfortunately, existing systems are not efficient in training MLLMs due to two obstacles.
%First, MLLM training recipe consists of multiple phases, each with distinct data mixture ratios across modalities.
%As shown in Figure~\ref{fig:intro}(a), early phases exclusively use text-only datasets; as training progresses, multimodal datasets such as image and video are incorporated.
%Moreover, in each phase, researchers often dynamically schedule data mixtures for algorithmic considerations, such as smoothly increasing the ratio of image data.
%These factors lead to dynamic relative workloads among modalities, which we quantify by defining \textit{modality ratio} as the proportion of modality-specific \textcolor{blue}{samples}.

% To quantify dynamic relative workloads among modalities (e.g., visual, auditory), we define \textit{modality ratio} as the proportion of modality-specific \textcolor{blue}{tokens}.
% For example, \textcolor{blue}{the image-text mixture ratio of XXX in Figure~\textcolor{blue}{xx} is XXX}.
% In addition, encoders and the LLM, as well as different encoders, exhibit heterogeneity in model architecture and size, further amplifying dynamic workloads across them.

%Second, for each modality, significant data skewness exhibits across and within diverse datasets, with up to \textcolor{blue}{XX} sample length variance observed in Figure~\ref{fig:intro}(b).
%When scaling to 10K GPUs, the skewness leads to dynamic workload distributions between \textcolor{blue}{encoders of the same modality}. 
%Specifically, each encoder is assigned samples with varying lengths, including some overlong outliers; some encoders may have no sample under insufficient workloads.
%Moreover, each encoder's output is embedded into LLM tokens, rendering the dynamic workloads between LLM microbatches. 

% \chunyu{Rethink ``coupling'' and ``decoupling'' resource allocation and parallelization.}

Current MLLM training systems fall short in handling dynamic workloads, as they statically couple resource allocation and model parallelization between encoders and the LLM backbone.
Some frameworks (e.g., Megatron-LM~\cite{megatron}) treat encoders as embedding layers of the LLM, allocating resources and parallelizing the entire MLLM in a unimodal manner using strategies such as pipeline parallelism (\S\ref{sec:basic}).
Consequently, when encoder workloads rise, the first LLM pipeline stage becomes a compute and memory bottleneck, leading to a $2.84\times$ throughput gap and out-of-memory (OOM) issues as shown in Figure~\ref{fig:intro}(c).
% Figure~\ref{fig:intro}(c) shows the training throughput of a Megatron-based 128-GPU task under dynamic workloads. 
% As observed, throughput exhibits significant variance for different image-text ratios and datasets, with up to $2.84\times$/$2.13\times$ throughput gap and out-of-memory (OOM) issues occured. 
Other systems (e.g., DistTrain~\cite{disttrain}) statically disaggregate encoders and the LLM backbone as two separate models, each with fixed, distinct resources and parallelism strategies.
Such disaggregation suffers from encoding bottlenecks when encoders are assigned excessive workloads, while inducing substantial device bubbles when encoders have insufficient samples.
% as they couple encoder-LLM resource allocation and parallelization as a monolithic decision. 
% Some frameworks (e.g., Megatron-LM~\cite{megatron}) treat encoders as data preprocessing layers of the first LLM pipeline stage, allocating resources and parallelizing in a unimodal manner.
% Other works (e.g., DistTrain~\cite{disttrain}) statically disaggregate encoders and the LLM as two separate models with distinct resources and parallelization. 
% Consequently, when encoder workloads increase, the first stage becomes a compute and memory bottleneck; when workloads decrease, encoder resources undergo prolonged idling due to insufficient samples. 
% Figure~\ref{fig:intro}(c) shows the training throughput of a Megatron-based 128-GPU task under dynamic workloads. 
% As observed, throughput exhibits significant variance for different image-text ratios and datasets, with up to $2.84\times$/$2.13\times$ throughput gap and out-of-memory (OOM) issues occured. 
Another recent work, Optimus~\cite{optimus}, decouples resource allocation and parallelization assuming static workloads, generating decisions solely from model information. 
Thus, it optimizes for each specific workload but fails to handle dynamic ones.



% Unlike traditional unimodal training, industrial-scale multimodal training features several distinct characteristics.
% First, modality encoders and the LLM backbone exhibit significant model size heterogeneity arising from different operator compositions. \NX{should say different modal encoders have different sizes, not the LLM vs encoder}. \NX{why OOM in figure4}
% % First, MLLMs exhibit significant heterogeneity in model size, as \textcolor{blue}{modality modules are typically smaller than the LLM backbone~\cite{qwen2-vl} (need rethink)}.
% Second, MLLM training builds upon a wide mixture of datasets spanning diverse modalities and task domains, each exhibiting distinct data lengths and distributions.
% % This data diversity drives the use of hybrid batching, which packs cross-modality sequences before batching, to mitigate zero padding~\cite{bytescale}.
% Lastly, MLLM training is divided into multiple phases, each with different configurations, such as LLM text-only pretraining and encoder-LLM image-text training.


% From our experience, industrial MLLM training demonstrates \textit{dynamic workloads} across encoders and the LLM, stemming from ever-changing mixture ratios of different modalities and task domains.
% Specifically, researchers typically employ multi-phase training recipes and intra-phase data scheduling, which dynamically adjust data proportions across modalities and task domains during the training process~\cite{internlm,qwen2.5-vl,internlm2}.
% Moreover, significant data skewness exhibits across modalities, datasets, and within individual datasets, with up to \textcolor{blue}{XX$\times$} sample length variation observed.
% When scaling to 10K GPUs, this skewness leads to dynamic load distribution across encoders and further induces dynamicity between LLM microbatches.
% % In addition, when scaling to 10K GPUs, \textcolor{blue}{load balancing between encoders becomes more dynamic} due to enlarged balancing scale and insufficient sequences within batches.



% From our experience, these characteristics induce workload dynamicity in MLLM training.
% Specifically, researchers typically employ multi-phase training recipes and intra-phase data scheduling, which dynamically adjust data proportions of different modalities and task domains during the training process~\cite{internlm,internlm2,qwen2-vl}.
% This dynamic mixture leads to resource underutilization when workloads decrease, resulting in up to \textcolor{blue}{XX\%} throughput drop.
% Moreover, significant data skewness exhibits across modalities, datasets, and within individual datasets, with up to \textcolor{blue}{XX$\times$} sequence length variation observed.
% This skewness adds further dynamicity while leading to load imbalance and pipeline bubbles with up to \textcolor{blue}{XX\%} throughput decrease.
% As a result, even with optimal parallelization, a \textcolor{blue}{XX-B} MLLM still experiences an average \textcolor{blue}{XX\%} throughput drop under dynamic workloads.



% Existing MLLM training systems encompass two typical schemes, neither of which efficiently handles dynamic workloads.
% The first is \textit{LLM-centric} scheme (e.g., Megatron-LM~\cite{megatron}), which treats encoders as data preprocessing layers of the first LLM pipeline stage and parallelizes the MLLM in a unimodal manner.
% While easy to engineer, this scheme suffers from imbalanced pipeline and poor scalability, as the first stage becomes a compute and memory bottleneck. 
% The second is \textit{disaggregation} scheme (e.g., DistTrain~\cite{disttrain}), which fully disaggregates encoders and the LLM through independent parallelization and resource allocation.
% This scheme enables flexible and scalable parallelization, yet is prone to resource underutilization when an encoder has insufficient workloads, given its statically over-provisioned resources.
% Moreover, disaggregation limits encoder resource quotas due to economic costs and resource contention with the LLM, which hinders scaling encoding concurrency via increased data parallelism (DP) replicas. \NX{there should be two highlighted high-level reasons why previous mllm frameworks do not work efficiently}


% The root cause of these limitations lies in treating model parallelization and resource allocation as an ``all-or-nothing'' decision.
% Specifically, existing schemes either tightly couple encoders with the LLM via shared parallelism strategies and resources, or fully disaggregate them as two models with separate parallelism strategies and resources. \NX{Not precise, the encoder only share the resource with the first pp stage?}
% As a result, when encoder workloads increase, LLM-centric scheme confronts heavier compute and memory bottleneck at the first stage; when workloads decrease, statically provisioned resources in disaggregation scheme suffer underutilization with increased bubbles.

Given the above limitations, an efficient system should decouple resource allocation and model parallelization, while adapting to dynamic workloads.
Specifically, by employing decoupled parallelism strategies, we can parallelize encoders with higher concurrency and more resources, i.e., with larger data parallelism (DP) degrees across all GPUs, to avoid bottlenecking LLM execution.
% by decoupling encoder-LLM parallelism strategies, we can parallelize encoders with high concurrency, such as with more data parallelism (DP), to avoid bottlenecking the LLM execution.
For the LLM, evidently, the ideal choice should be inheriting all full-fledged parallelization techniques from unimodal training~\cite{megatron-scale,zerobubble,flux}.
Meanwhile, by colocating encoders and the LLM across GPUs, we can temporally orchestrate their execution and reactively adapt their elapsed times in response to workload shifts.
% and jointly orchestrating their execution, we can temporally sharing resources and \textcolor{blue}{reactively adapting their elapsed times} in response to workload shifts.
% improve resource utilization and ensure workload resilience via temporally sharing resources and \textcolor{blue}{reactively adapting their elapsed times} in response to workload shifts.
These design considerations constitute the key insight of this paper, which we refer to as \textit{encoder-LLM multiplexing}.
% There are three major challenges to 

On top of this training scheme, we build \textbf{\sysname{}}, a MLLM training system for dynamic workload adaption and hyper-scale deployment.
\sysname{} consists of three key innovations to train a production-grade MLLM with high efficiency, scalability, and engineering flexibility.

\begin{itemize}
[label={$\triangleright$}, itemsep=0pt, parsep=0pt, labelsep=5pt, leftmargin=*, topsep=3pt,partopsep=0pt]
% [itemsep=0pt, parsep=0pt, labelsep=5pt, leftmargin=*, topsep=3pt,partopsep=0pt]
\itemsep3pt

\item First, \sysname{} decouples parallelization between encoders and the LLM backbone with tailored strategies for variable-length, long-context workloads and hyper-scale deployment.
For encoders, \sysname{} proposes long-short sequence parallelism, which unifies DP, Ulysses SP, and ZeRO2/3 to process variable-length samples simultaneously.
For the LLM, \sysname{} incorporates full-fledged 5D parallelism with a communication-efficient layout to mitigate execution interference.

\item Second, \sysname{} proposes unified encoder-LLM representations to enable flexible, extensible colocation across GPU ranks.
This is motivated by the distinct parallelism strategies and intricate data dependencies between encoders and the LLM, which prevent simply wrapping encoders as LLM layers or nestedly inserting encoder operations into LLM codes in codebases.
The ideas behind is to abstract encoders as anchors to the LLM pipeline, while encapsulating complex parallelization and communication details.
Building on representations, \sysname{} proposes a new paradigm of encoder-LLM joint pipeline, featuring uniform, on-demand encoder insertion to maintain structural stability under dynamic workloads.
% employing uniform, on-demand encoder insertion to maintain structural stability under dynamic workloads.

\item Lastly, \sysname{} proposes multiple techniques to optimize workload balance under multimodal data and hyper-scale parallelization.
For skewed dataset distributions, \sysname{} employs grouped reordering in decentralized data loaders to balance workloads across encoders.
When resharding multimodal embeddings from encoder to LLM ranks, \sysname{} balances workloads across LLM ranks and mitigates communication stragglers via adaptive sample sharding and symmetric dispatching.

\end{itemize}

% Specifically, to mitigate pipeline imbalance, the system decouples parallelism strategies for encoders and the LLM.
% Encoders should be parallelized with high concurrency to avoid bottlenecking LLM execution.
% For the LLM, the ideal way is to inherit all full-fledged parallelism strategies from unimodal pretraining~\cite{llama3}, such as highly optimized pipeline~\cite{megatron-scale,pipedream} and tensor parallelism (TP)~\cite{megatron,flux}.
% Moreover, to improve resource utilization, the system colocates encoders and the LLM to multiplex resources, while jointly orchestrating encoder-LLM execution for workload resilience.
% High-level model representations are required to hide the colocation complexities, such as encoder-LLM data dependencies under decoupled parallelization. 
% These design considerations constitute the key insight of this paper, which we refer to as \textbf{\textit{encoder-LLM multiplexing}}.
% There are three major challenges to architect a foundational system based on this multiplexing-based scheme.

% The first challenge is to determine parallelism strategies for encoders and the LLM under long contexts and hyper-scale.
% To inherit full-fledged parallelism strategies for the LLM, encoder parallelization should not interfere with the LLM execution.
% For instance, it cannot constrain the selection of LLM parallelism strategies or bottleneck the LLM pipeline.
% Moreover, static encoder parallelization falls short in handling samples with varying lengths.
% Long-context samples require to be processed with sequence parallelism (SP) to avoid OOM issues, while processing short samples with SP leads to GPU underutilization.

% The second challenge is encoder-LLM colocation and orchestration with workload resilience.
% Encoders and the LLM share distinct parallelism strategies, intricate data dependencies, and \textcolor{blue}{isolated implementations}, making it non-trivial for colocation.
% For instance, nestedly inserting encoder parallelization and communication codes into LLM pipeline functions is not allowed to avoid \textcolor{blue}{code pollution}.
% High-level model representations are required to hide colocation complexities and be extensible to different algorithms.
% Building on representations, designing a joint encoder-LLM orchestration that balances efficiency, workload resilience, and \textcolor{blue}{ease of use} remains unexplored.

% The third challenge is workload balancing for encoders and the LLM.
% To alleviate dataset skewness during data loading, a natural approach is globally reordering modality samples across encoders.
% This incurs substantial communication overhead at hyper-scale.
% Moreover, encoders and the LLM execute many-to-many data transmission to exchange embeddings or gradients, such as from encoder data parallelism (DP) ranks to LLM context parallelism (CP) ranks.
% This transmission includes resharding multimodal samples and dispatching to multiple ranks, thus prone to communication stragglers and workload imbalance across destination ranks. 
% % \NX{lost on the third challenge}


% Therefore, an efficient, \textit{workload-resilient} system should decouple model parallelization and resource allocation in MLLM training. 
% To mitigate pipeline imbalance and enhance scalability, the system decouples parallelism strategies of encoders and the LLM, while distributing encoders across all LLM ranks for colocation --- rather than dedicated ranks or those of the first LLM stage.
% To improve resource utilization, instead of static over-provisioning, the system jointly orchestrates interleaved encoder-LLM execution for resource multiplexing, and \textcolor{blue}{uniformly inserts encoders across stages for workload resilience based on the observation in \S\ref{sec:pipeline}}.
% These design considerations constitute the key insight of this paper, which we refer to as \textbf{\textit{encoder-LLM multiplexing}}.
% There are two major challenges to architect a foundational system based on this multiplexing-based scheme.

% At the model level, enabling efficient, scalable encoder-LLM co-execution with system flexibility and workload resilience is non-trivial.
% Given encoder-LLM heterogeneity, efficient parallelization requires adaptively determining their hybrid parallelism strategies based on model and data scales. 
% Obviously, the multiplexing scheme adds more engineering complexities to the encoder-LLM colocation.
% Therefore, high-level model representations are necessary to reduce engineering effort and generalize across diverse algorithms.
% Moreover, designing a joint encoder-LLM execution schedule with workload resilience remains unexplored.



% \chunyu{Complex v.s. industrial-grade flexibility and minimal engineering effort.}
% \chunyu{Industrial-grade systems typically adhere to the design philosophy of simplicity.}
% \chunyu{Multiplexing-based encoder-LLM co-orchestration is complex. How to determine decoupled parallelism strategies and colocate encoders and the LLM, improving efficiency and scalability, while ensuring transparent integration with minimal engineering effort? How to architect an encoder-LLM execution schedule that not only mitigates pipeline imbalance, reduces resource bubbles, and satisfies data dependencies, but also being resilient to workload dynamicity, and compatible to existing LLM optimizations.}


% At the data level, hyper-scaled, decentralized load balancing across all ranks under dynamic workloads is non-trivial.
% As mentioned, dynamic data mixtures lead to load imbalance for both encoders and the LLM.
% At hyper-scale, the expanded balancing scale and more skewed modality data further exacerbate this imbalance.
% Unlike prior systems that only load data on the first stage~\cite{megatron,dynapipe}, the multiplexing scheme distributes encoders across all ranks and requires decentralized data loading.
% This makes load balancing more challenging, as token-based global reordering incurs sustantial communication overhead at hyper-scale (\S\ref{sec:reorder}). 


% \chunyu{The dynamic modality data mixture causes load imbalance on both encoders and the LLM.}
% \chunyu{When scaling to 10K GPUs, the enlarged balancing scale and longer modality data further aggrevates the imbalance.}
% \chunyu{Unlike prior works that only perform data loading on PP0, the multiplexing scheme brings decentralized data loading across all ranks.}
% \chunyu{This makes global load balancing more challenging, as global reordering and XXX incurs substantial overhead at hyper-scale.}
% \chunyu{A }


% \chunyu{Achieving global load balancing under the multiplexing scheme (disributed on all ranks, unlike prior works only on PP0) is non-trivial. The workload dynamicity incurs imbalanced encoder computations at hyper-scale (\S\ref{sec:imbalance_analysis}), which cannot be resolved by naive global reordering, which incurs substantial overhead at hyper-scale because all data loaders are decentralized across all ranks. Larger DP world size, longer modality data, or changed modality mixture further aggrevates the imbalance. }




% An intuitive approach is to 
% \chunyu{select one of the two schemes based on model size and workloads, but they share different implementations...}


% To address these challenges, we present \textbf{\sysname{}}, a workload-resilient system for hyper-scaled MLLM training.
% \sysname{} consists of three key innovations to achieve efficiency, scalability, and engineering flexibility.

% \begin{itemize}
% [label={$\triangleright$}, itemsep=0pt, parsep=0pt, labelsep=5pt, leftmargin=*, topsep=3pt,partopsep=0pt]
% % [itemsep=0pt, parsep=0pt, labelsep=5pt, leftmargin=*, topsep=3pt,partopsep=0pt]
% \itemsep3pt

%     % \item Based on in-depth parallelism analysis from the industrial perspective, \sysname{} proposes \textcolor{blue}{long-short sequence parallelism}, which unifies data parallelism (DP), ZeRO2/3, and Ulysses SP for scalable, long-context encoder parallelization. 
%     % Given dynamic workloads, it temporarily shifts node states across parallelism strategies to process variable-length samples via intra-microbatch sample reordering and bucket-based dataset profiles. 
%     % For the LLM, \sysname{} incorporates full-fledged 5D parallelism strategies and advanced optimizations, such as virtual pipeline and TP communication overlap.
%     % % through a \textcolor{blue}{configuration interface}. \NX{not clear}

%     % \item \sysname{} proposes an unified encoder-LLM representation to enable transparent, extensible colocation and joint workload-resilient orchestration. 
%     % The idea behind is to abstract modality-specific encoders as anchors to the LLM pipeline in a SPMD-aware manner.
%     % By encapsulating parallelization, algorithmic implementations, and data transmission, this representation exposes high-level APIs for flexible encoder-LLM colocation. 
%     % Building on representations, \sysname{} provides two foundamental \textcolor{blue}{guidelines} on workload-resilient pipeline, including uniform, on-demand encoder insertion across LLM pipeline stages and dependency-aware anchor size determination.
    
%     % \item \sysname{} proposes decentralized grouped reordering to balance encoder workloads within global batches while reducing communication overhead. 
%     % For workload balancing in encoder-LLM data transmission, \sysname{} employs \textcolor{blue}{selective intra-sample sharding} and \textcolor{blue}{dual-step data dispatching} to propagate encoded tokens and gradients of different modalities between encoder and LLM ranks.

% \end{itemize}

\sysname{} has been deployed as the foundation for most large-scale MLLM training tasks in our company, scaling to thousands of GPUs. 
Extensive experiments demonstrate that \sysname{} improves training throughput by $1.27\times$--$7.57\times$ under dynamic multimodal workloads across various model and hardware scales, compared to four state-of-the-art baselines.
We also share our practical operational experience of deploying \sysname{} at hyper-scale, including performance analysis, MFU optimizations, and solutions to engineering failures.



% To address these limitations, we propose \textbf{\sysname{}}, a workload-resilient system for hyper-scaled MLLM training.
% Given that tightly coupled and fully disaggregated schemes both lead to potential inefficiencies, \sysname{} unifies the strengths of both by logically decoupling encoder-LLM parallelization, while physically colocating on shared compute resources. 
% On this basis, the above issues are mitigated via fine-grained model orchestration and load scheduling.
% We refer to this insight as \textbf{\textit{encoder-LLM multiplexing}}.
% Obviously, this multiplexing scheme complicates encoder-LLM co-execution, not to mention the inherent algorithmic and engineering complexities of industrial LLMs. 
% % which hinder ad-hoc encoder integration.
% % While multiplexing complicates encoder-LLM co-execution, we find that workload dynamicity only affect encoders, whereas the LLM remains stable due to uniform sequence lengths in hybrid batching.
% % Moreover, industrial LLMs exhibit algorithmic and infrastructural complexities, which hinders case-specific encoder integration.
% Our second insight, therefore, is \textbf{\textit{transparent integration}} of encoders into the native LLM execution schedule, without intrusive modifications to its implementation or execution.
% % These observations motivate us to integrate encoders into the native LLM workflow without intrusive effects, which we term as \textbf{\textit{transparent integration}}.

% Building on these insights, \sysname{} architects a foundational framework to improve training efficiency under dynamic workloads, while supporting MLLMs of varying scales and diverse encoders.
% Moreover, \sysname{} facilitates flexible algorithm customization with minimal engineering effort, while being compatible with existing optimizations (e.g., communication overlap~\cite{flux}).
% These design considerations pose two critical challenges.




% \chunyu{We wish that: once the MLLM system has been deployed, no matter how dynamic workloads, always efficient and under-controlled (since reconfig a MLLM system is extremely labor-intensive at hyper-scale).}


==> sections/relatedwork.tex <==
\section{Related Work}

%\subsection{Hello World}
